Unintentional Unalignment: Likelihood Displacement in Direct Preference Optimization

Direct Preference Optimization (DPO) and its variants are increasingly used for aligning language models with human preferences. Although these methods are designed to teach a model to generate preferred responses more frequently relative to dispreferred responses, prior work has observed that the likelihood of preferred responses often decreases during training. The current work sheds light on the causes and implications of this counter-intuitive phenomenon, which we term likelihood displacement. We demonstrate that likelihood displacement can be catastrophic, shifting probability mass from preferred responses to responses with an opposite meaning. As a simple example, training a model to prefer $\texttt{No}$ over $\texttt{Never}$ can sharply increase the probability of $\texttt{Yes}$. Moreover, when aligning the model to refuse unsafe prompts, we show that such displacement can unintentionally lead to unalignment, by shifting probability mass from preferred refusal responses to harmful responses (e.g., reducing the refusal rate of Llama-3-8B-Instruct from 74.4% to 33.4%). We theoretically characterize that likelihood displacement is driven by preferences that induce similar embeddings, as measured by a centered hidden embedding similarity (CHES) score. Empirically, the CHES score enables identifying which training samples contribute most to likelihood displacement in a given dataset. Filtering out these samples effectively mitigated unintentional unalignment in our experiments. More broadly, our results highlight the importance of curating data with sufficiently distinct preferences, for which we believe the CHES score may prove valuable.

==> app_scratch_plots_tables.tex <==
\clearpage

\section{Plots and Tables}
%TODO make these prettier
\begin{minipage}{\linewidth}
  \centering
  \begin{minipage}[b][][b]{0.45\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figs/sorrybench/refusal_rates_train.pdf}
          
          \label{fig:refusalrate}
          \caption{\emph{Catastrophic likelihood displacement on SORRY-Bench}: Performing DPO on the on-policy data results in a dramatic decrease in the model tendency to refuse answers to toxic or harmful prompts, as our theory predicts. Adding an SFT term or only retaining the least dissimilar pairs alleviates the issue.}
      \end{figure}
  \end{minipage}
  \hspace{0.035\linewidth}
  \begin{minipage}[b][][b]{0.5\linewidth}
        \begin{table}[H]
\scalebox{0.75}{
\begin{tabular}{lcc}
\toprule
\multicolumn{3}{c}{\hspace{15mm}\textbf{Change in Preferred Response Log Probability}}\\ \cmidrule{2-3}
\multicolumn{1}{r}{} & Gemma-2B-IT & Llama-3-8B-Instruct \\ \midrule \\[-0.9em]
DPO & $-59.2 \pm$ \footnotesize{$5.3$} & \hspace{1mm} $-48.1 \pm$ \footnotesize{$22.1$} \\[0.15em]
DPO (filtered) & $-45.7 \pm$ \footnotesize{$2.5$} & $-27.7 \pm$ \footnotesize{$2.7$} \\[0.15em]
DPO (gold) & $+ 54.6 \pm$ \footnotesize{$3.2$} & $+ 24.9 \pm$ \footnotesize{$3.0$} \\[0.15em]
DPO + SFT & $+ 20.2 \pm$ \footnotesize{$2.4$} & $+ 28.6 \pm$ \footnotesize{$0.3$} \\[0.1em]
\bottomrule
\end{tabular}}
\label{tab:llchange}
\caption{The change in the log-likelihood of the preferrred responses with DPO on SorryBench with on-policy responses, DPO on a version of the dataset filtered using the CHES score, DPO on the dataset with gold responses, and DPO with an additional SFT term (coefficient $= 1$). For the filtered dataset, we keep the top 5\% of pairs where the preferred and dispreferred pairs are most different according to the CHES score.}
        \end{table}
  \end{minipage}
\end{minipage}

\begin{minipage}{\linewidth}
  \centering
  \begin{minipage}[b][][b]{0.45\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figs/sorrybench/refusal_rates_train.pdf}
          \label{fig:refusalrate_backup}
          \caption{\emph{Catastrophic likelihood displacement on SORRY-Bench}: Performing DPO on the on-policy data results in a dramatic decrease in the model tendency to refuse answers to toxic or harmful prompts, as our theory predicts. Adding an SFT term or only retaining the least dissimilar pairs alleviates the issue.}
      \end{figure}
  \end{minipage}
  \hspace{0.02\linewidth}
  \begin{minipage}[b][][b]{0.44\linewidth}
\begin{figure}[H]
\includegraphics[width=\linewidth]{figs/sorrybench/legend-3-TTO.pdf}\\
\hspace*{-0.06\linewidth}          \includegraphics[width=1.1\linewidth]{figs/sorrybench/sp_p_.pdf}
          \label{fig:sorrybench_ches_category_backup}
          \caption{The length-normalized CHES values of the various pairs in the SorryBench dataset, as measured with Llama-3-8B-Instruct. The score distinguishes examples with one refusal and one non-refusal--- with a high CHES score, and those with two refusals or two non-refusals, usually with a lower CHES score.}
      \end{figure}
  \end{minipage}
\end{minipage}

\begin{minipage}{\linewidth}
  \centering
  \begin{minipage}[b][][b]{0.45\linewidth}
      \begin{figure}[H]
          \includegraphics[width=\linewidth]{figs/sorrybench/refusal_rates_ipo_train.pdf}
          \label{fig:refusalrate_}
          \caption{\emph{Catastrophic likelihood displacement on SORRY-Bench}: Performing IPO on the on-policy data results in a dramatic decrease in the model tendency to refuse answers to toxic or harmful prompts, as our theory predicts. Adding an SFT term or only retaining the least dissimilar pairs alleviates the issue.}
      \end{figure}
  \end{minipage}
  \hspace{0.035\linewidth}
  \begin{minipage}[b][][b]{0.5\linewidth}
        \begin{table}[H]
\scalebox{0.75}{
\begin{tabular}{lcc}
\toprule
\multicolumn{3}{c}{\hspace{15mm}\textbf{Change in Preferred Response Log Probability}}\\ \cmidrule{2-3}
\multicolumn{1}{r}{} & \textbf{Gemma-2B-IT} & \textbf{Llama-3-8B-Instruct} \\ \midrule
IPO & \hspace{2.1mm}-$73.4 \pm 11.5$ & \hspace{1.3mm}-$65.9 \pm 18.5$ \\
IPO (filtered) & \hspace{0.8mm}-$45.9 \pm 1.1$ & \hspace{0.5mm}-$29.2 \pm 3.1$ \\
IPO (gold) & +$27.4 \pm 6.6$ & +$26.2 \pm 3.5$ \\
IPO + SFT & +$10.1 \pm 3.7$ & +$20.3 \pm 3.1$ \\
\bottomrule
\end{tabular}}
\label{tab:llchange_ipo}
\caption{The change in the log-likelihood of the preferrred responses with IPO on SorryBench with on-policy responses, IPO on a version of the dataset filtered using the CHES score, IPO on the dataset with gold responses, and IPO with an additional SFT term (coefficient $= 100$). For the filtered dataset, we keep the top 5\% of pairs where the preferred and dispreferred pairs are most different according to the CHES score.}
        \end{table}
  \end{minipage}
\end{minipage}

% \begin{figure}[H]
% \centering
% \includegraphics[width=\linewidth]{figs/similarity/legend-3-CEL.pdf}\\
% \vspace*{-0.5em}
% \subfloat[OLMo-1B]{
% \includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_olmo1b_sft_dpo.pdf}
% }
% \hspace*{-1em}
% \subfloat[Gemma-2B]{
% \includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_gemma_2b_sft_dpo.pdf}
% }
% \hspace*{-1em}
% \subfloat[Llama-3-8B]{
% \includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_llama-3-8b_sft_dpo.pdf}
% }
% \caption{Change in the log-likelihood of preferred responses with 512 examples at varying percentiles of different measures. We report results with three models when performing DPO on UltraFeedback. We see that the CHES measures correlates well with amount of likelihood displacement, while Edit Distance and Last Hidden Embedding Similarity show less or no correlation. We also found that token overlap performs similarly to CHES.}
% \label{fig:llplot}
% \end{figure}

% \begin{table}[H]
% \centering
% \begin{tabular}{rcc}
% \toprule
% \multicolumn{3}{c}{\textbf{$\Delta$(Log-probability of Preferred Response)}}\\ \cmidrule{2-3}
% \multicolumn{1}{r}{} & \textbf{Gemma-2B-IT} & \textbf{Llama-3-8B-Instruct} \\ \midrule
% DPO & -60.3 & -70.1 \\
% DPO (filtered data) & -46.6 & -24.6 \\
% DPO (gold data) & 53.0 & 28.3 \\
% DPO + SFT & 19.9 & 28.7 \\
% \bottomrule
% \end{tabular}
% \label{tab:llchange}
% \caption{The change in the log-likelihood of the preferrred responses with DPO on the entire dataset with on-policy responses, DPO on a version of the dataset filtered using the CHES score, DPO on the dataset with gold responses, and DPO with an additional SFT term (coefficient $= 1$). For the filtered dataset, we keep the top 5\% of pairs where the preferred and dispreferred pairs are most different according to the CHES score.}
% \end{table}

% \begin{wrapfigure}{r}{0.6\textwidth} 
%   \centering
%   \includegraphics[width=\linewidth]{figs/sorrybench/refusal_rates_train.pdf}
  
%   \label{fig:refusalrate}
%   \caption{\emph{Catastrophic displacement on SORRY-Bench}: Performing DPO on the on-policy data results in a dramatic decrease in the model tendency to refuse answers to toxic or harmful prompts, as our theory predicts. Adding an SFT term or only retaining the least dissimilar pairs alleviates the issue.}
% \end{wrapfigure}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figs/similarity/legend-3-CEL.pdf}\\
\vspace*{-0.5em}
\subfloat[OLMo-1B]{
\includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_olmo1b_sft_dpo.pdf}
}
\hspace*{-1em}
\subfloat[Gemma-2B]{
\includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_gemma_2b_sft_dpo.pdf}
}
\hspace*{-1em}
\subfloat[Llama-3-8B]{
\includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_llama-3-8b_sft_dpo.pdf}
}
\caption{Change in the log-likelihood of preferred responses with 512 examples at varying percentiles of different measures. We report results with three models when performing DPO on UltraFeedback. We see that the CHES score correlates well with the amount of likelihood displacement, while Edit Distance and Last Hidden Embedding Similarity show less or no correlation. We report results with three seeds.
}
\label{fig:llplot}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figs/similarity/legend-3-CEL.pdf}\\
\vspace*{-0.5em}
\subfloat[OLMo-1B]{
\includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_olmo1b_sft_ipo.pdf}
}
\hspace*{-1em}
\subfloat[Gemma-2B]{
\includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_gemma_2b_sft_ipo.pdf}
}
\hspace*{-1em}
\subfloat[Llama-3-8B]{
\includegraphics[height=0.23\linewidth]{figs/similarity/ultrafeedback_llama-3-8b_sft_ipo.pdf}
}
\caption{Change in the log-likelihood of preferred responses when using IPO instead of DPO. Other settings are the same as in Figure~\ref{fig:llplot}. We see that CHES is by far the most informative measure even with IPO.}
\label{fig:llplot2}
\end{figure}








==> app_sign_gf.tex <==
\section{Analysis of Likelihood Displacement for Adaptive Optimizers}
\label{app:sign_gf}

\todo{
Extension of analysis to sign gradient flow, which captures adaptive optimizers such as Adam and RMSProp in the limit of small learning rate~\cite{ma2020qualitative,malladi2023kernel}.
}
